POSTCONDBENCH: Benchmarking Correctness and Completeness in Formal Postcondition Inference

Formal postconditions precisely characterize program behavior and support debugging, testing, and verification, but writing them requires substantial expertise and effort. This has motivated recent work on automatically generating postconditions from code and natural-language artifacts using large language models (LLMs). However, evaluation remains a key bottleneck. Existing benchmarks primarily emphasize correctness under limited evaluation settings, often relying on surface-form matching or manual assessment on small or synthetic datasets. We introduce POSTCONDBENCH, a multilingual benchmark for evaluating method-level postcondition generation from real-world software. POSTCONDBENCH comprises 420 Python and Java tasks drawn from 121 open-source projects, each paired with a high-quality ground-truth postcondition set constructed with expert involvement. To enable automatic evaluation, POSTCONDBENCH provides a runnable execution environment and operationalizes completeness via defect discrimination: a postcondition set is more complete if it is violated by more defective implementations while remaining satisfied on correct executions. Using POSTCONDBENCH, we formulate three generation settings and evaluate five SOTA LLMs. Our results reveal a substantial gap between correctness and completeness, and show that repository-level dependencies and method complexity exacerbate this gap.

==> src/exp_setting/metrics.tex <==
\subsection{Metrics} 

We use Pass@k-like metrics \cite{chen2021evaluating} to assess correctness and completeness. 
We also define a complete-to-correct ratio (C2C) to assess the gap between correctness and completeness.

\paragraph{Correctness and completeness}
The Pass@k metric assesses the expectation of at least one solution appearing among k generated candidates for a given problem.
In our experiments, for a method $m$, we generate $n$~postcondition sets and evaluate their correctness and completeness.
We set:
\begin{align*}
    c_{corr} & = \sum_{i=1}^n \ind[\corrCond(m, p_i)] \text{ and} \\
    c_{comp} & = \sum_{i=1}^n \ind[\cevalCond(m, p_i)],
\end{align*}
in which $\ind$~denotes the indicator function.
In our experiments, we generate five postcondition sets for each target method (i.e., $n=5$). 
Then we set:
\begin{align*}
    \text{Corr@k} & = \expectation( 1 - \tbinom{n - c_{corr}}{k} / \tbinom{n}{k} ) \text{ and}\\
    \text{Comp@k} & = \expectation( 1 - \tbinom{n - c_{comp}}{k} / \tbinom{n}{k} ).
\end{align*}

\paragraph{Complete-to-correct ratio}
We use the complete-to-correct ratio (C2C) to assess the ratio of a correct postcondition set being complete.
Considering all generated postcondition sets in an experiment, each has a correctness and a completeness evaluation result (note that a complete postcondition set must be correct), we set:
\[
\text{C2C} = \frac{\text{Number of Complete Postcondition Sets}}{\text{Number of Correct Postcondition Sets}}
\]
A lower complete-to-correct ratio demonstrates a larger gap between a postcondition set being correct and complete.

